Future prospects

This chapter addresses limitations to current 21-cm signal detection instruments, being related to the instrument, environment, signal processing or science, and what lies beyond the current horizon for 21-cm science, especially in the 2030s and beyond. We address how to overcome current challenges and drive the field forward, not only approaching a detection of the 21-cm signal but to a full characterisation of its parameterspace, in particular, probing an increasingly larger volume of k-modes (spatially and in redshifts). We also will shortly touch upon the kinds of questions that could drive such future endeavours.

==> compile_pdflatex <==
pdflatex ms
bibtex Furlanetto/chapter
bibtex Mirocha/chapter
bibtex Greig/chapter
bibtex Bernardi/chapter
bibtex Chapman_Jelic/chapter
bibtex Greenhill_Subrahmanyan/chapter
bibtex Trott_Pober/chapter
bibtex Koopmans_Bernardi/chapter
pdflatex ms
pdflatex ms
rm *~ *.aux *.log *.blg *.out *\#
